Vision-Assisted User Clustering for Robust mmWave-NOMA Systems

When operated in the mmWave band, user channels get highly correlated which can be exploited in mmWave-NOMA systems to cluster a set of "correlated" users together. Identifying the set of users to cluster greatly affects the viability of NOMA systems. Typically, only channel state information (CSI) is used to make these clustering decisions. When any problem arises in accessing up-to-date and accurate CSI, user clustering will not properly function due to its hard-dependency on CSI, and obviously, this will negatively affect the robustness of the NOMA systems. To improve the robustness of the NOMA systems, we propose to utilize emerging trends such as location-aware and camera-equipped base stations (CBSs) which do not require any extra radio frequency resource consumption. Specifically, we explore three different dimensions of feedback that a CBS can benefit from to solve the user clustering problem, namely CSI-based feedback and non-CSI-based feedback, comprised of user equipment (UE) location and the CBS camera feed. We first investigate how the vision assistance of a CBS can be used in conjunction with other dimensions of feedback to make clustering decisions in various scenarios. Later, we provide a simple user case study to illustrate how to implement vision-assisted user clustering in mmWave-NOMA systems to improve robustness, in which a deep learning (DL) beam selection algorithm is trained on the images captured by the CBS to perform NOMA clustering. We demonstrate that user clustering without CSI can achieve comparable performance to accurate CSI-based solutions, and user clustering can continue to function without much performance loss even in the scenarios where CSI is severely outdated or not available at all.

==> ResNet18Details.tex <==
\subsection{ResNet-18 beam Prediction}

Learning beam prediction from images is essentially an image classification task, where the algorithm relies on knowing the user's location on the scene. The set of candidate beam vectors divide the scene (spatial dimensions) into multiple sectors. Depending on the user location in the scene, which is known to the algorithm, the goal of the algorithm is then to identify to which of the sectors a user belongs. In other words, we want to find the users "best beam direction". To put it mathematically, we want to select the best beam $f^*$ from set of candidate beams $F$. Let $\mathbf{h}$ represent the channel info for the user.

\begin{equation}
    f^* = \underset{\mathbf{f} \in F}{\textrm{argmax}} ~\mathbb{E}[\Vert\mathbf{h}^T \mathbf{f}\Vert_2^2]
\end{equation}

The approach used in the paper to learn the beam prediction function is based on deep convolutional neural networks and transfer learning. A pre-trained Resnet-18 network trained on the popular ImageNet2012 dataset is customized for the beam-prediction problem. The final fully connected layer in ResNet-18 is removed and replaced with another fully connected layer of 64 neurons to represent the 64 beams. Using training data of images of users explicitly marked against their best beam, in a supervised learning setting, the model learns a new classification function, $f_\Theta(X)$, that maps an image to a beam index. Thus, the beam prediction function $f_\Theta(X)$, parameterized by a set of parameters $\Theta$; outputs a probability distribution $P = \{p_0, ..., p_{63}\}$. The best beam corresponds to the index of the element with maximum probability, $\mathbf{\hat{f} = f_{j^*}}$, where

\begin{equation}
    j^* = \underset{j \in \{0,..,63\}}{\textrm{argmax}} \{p_0, .., p_{63}\}.
\end{equation}
The parameters of the neural network are tuned so that we can maximize the probability that $\mathbf{\hat{f}} = \mathbf{f^*}$, i.e., $f_\Theta(X)$ chosen to maximize $P(\mathbf{\hat{f}} = \mathbf{f^*}|X)$.

==> glossaries.tex <==
\newacronym{SA}{SA}{Simulated Annealing}
\newacronym{VLC}{VLC}{visible light communications}
\newacronym{RF}{RF}{radio frequency}
\newacronym{V2V}{V2V}{vehicle-to-vehicle}
\newacronym{V2X}{V2X}{vehicle-to-everything}
\newacronym{B5G}{B5G}{beyond-fifth generation}
\newacronym{5G}{5G}{fifth-generation}
\newacronym{6G}{6G}{sixth-generation}
\newacronym{LED}{LED}{light emitting diode}
\newacronym{LEDs}{LEDs}{light emitting diodes}
\newacronym{OMA}{OMA}{orthogonal multiple access}
\newacronym{FDMA}{FDMA}{frequency-division multiple-access}
\newacronym{TDMA}{TDMA}{time-division multiple-access}
\newacronym{CDMA}{CDMA}{code-division multiple-access}
\newacronym{OFDMA}{OFDMA}{orthogonal frequency-division multiple-access}
\newacronym{WDMA}{WDMA}{wavelength-division multiple-access}
\newacronym{NOMA}{NOMA}{Non-orthogonal multiple access}
\newacronym{PD-NOMA}{PD-NOMA}{power-domain NOMA}
\newacronym{SC}{SC}{superposition coding}
\newacronym{SIC}{SIC}{successive interference cancellation}
\newacronym{BS}{BS}{base station}
\newacronym{QoS}{QoS}{quality-of-service}
\newacronym{NP}{NP}{non-deterministic polynomial-time}
\newacronym{DCO-OFDM}{DCO-OFDM}{direct-current biased optical-OFDM}
\newacronym{ITU}{ITU}{international telecommunication union}
\newacronym{FoV}{FoV}{field-of-view}
\newacronym{FoVs}{FoVs}{field-of-views}
\newacronym{CSI}{CSI}{channel state information}
\newacronym{LACO-OFDM}{LACO-OFDM}{layered asymmetrically clipped optical OFDM}
\newacronym{FR}{FR}{frequency reuse}
\newacronym{EAs}{EAs}{evolutionary algorithms}
\newacronym{C-LiAN}{C-LiAN}{centralized light access network}
\newacronym{AP}{AP}{access point}
\newacronym{APs}{APs}{access points}
\newacronym{PD}{PD}{photo-diode}
 \newacronym{PDs}{PDs}{photo-diodes}
\newacronym{SINR}{SINR}{signal-to-noise-interference ratio}
\newacronym{LoS}{LoS}{line-of-sight}
\newacronym{AWGN}{AWGN}{additive white Gaussian noise}
\newacronym{SNR}{SNR}{signal-to-noise ratio}
\newacronym{NLUPA}{NLUPA}{next-largest-difference user-pairing algorithm}
\newacronym{D-NLUPA}{D-NLUPA}{divide-and-next-largest-difference user-pairing algorithm}
\newacronym{NAICS}{NAICS}{network-assisted interference cancellation and suppression}
\newacronym{LTE}{LTE}{long term evolution}
\newacronym{3GPP}{3GPP}{3rd Generation Partnership Project}
\newacronym{CR}{CR}{cognitive radio}
\newacronym{2D}{2D}{two-dimension}
\newacronym{GP}{GP}{gradient projection}
\newacronym{umMTC}{umMTC}{ultra-massive machine-type communication}
\newacronym{IoE}{IoE}{internet-of-everything}
\newacronym{ZF}{ZF}{zero-forcing}
\newacronym{NLIP}{NLIP}{non-linear integer programming}
\newacronym{DP}{DP}{dynamic programming}
\newacronym{THz}{THz}{Terahertz}
\newacronym{D2D}{D2D}{device-to-device}
\newacronym{mmWave}{mmWave}{Millimeter-wave}
\newacronym{PS}{PS}{phase shifter}
\newacronym{PA}{PA}{power amplifier}
\newacronym{ABF}{ABF}{analog beamforming}
\newacronym{SPS}{SPS}{single-phase shifter}
\newacronym{AWV}{AWV}{antenna weight vector}
\newacronym{EE}{EE}{energy efficiency}
\newacronym{SE}{SE}{spectral efficiency}
\newacronym{NLoS}{NLoS}{non-line-of-sight}
\newacronym{mMIMO}{mMIMO}{massive multiple-input multiple-output}
\newacronym{MISO}{MISO}{multiple-input-single-output}
\newacronym{SISO}{SISO}{single-input single-output}
\newacronym{MOO}{MOO}{multi-objective optimization}
\newacronym{HP}{HP}{hybrid beamforming}
\newacronym{SCA}{SCA}{successive convex approximation }
\newacronym{SOC}{SOC}{second order cone}
\newacronym{RHS}{RHS}{right-hand side}
\newacronym{SDR}{SDR}{semidefinite relaxation}
\newacronym{VR}{VR}{virtual reality}
\newacronym{XR}{XR}{augmented reality}
\newacronym{NR}{NR}{new radio}
\newacronym{FD}{FD}{full-duplex}
\newacronym{QoE}{QoE}{quality-of-experience}
\newacronym{ULA}{ULA}{uniform linear array}
\newacronym{SI}{SI}{self-interference}
\newacronym{DF}{DF}{decode-and-forward}
\newacronym{GEE}{GEE}{global energy efficiency}
\newacronym{CNOMA}{CNOMA}{cooperative NOMA}

==> thikningNotes.tex <==
Different Clustering Approaches: 
\begin{enumerate}
    \item Approach-1: ch. info + user location (cos similarity metric)
    \item Approach-2: user location only (K-means clustering)
    \item Approach-3: BS images + user locations (proposed approach here).  
\end{enumerate}


 \begin{itemize}
     \item  Take a picture with multiple users. With location information known, simply "put a car" image there where there is a user and then it becomes the same problem as the "beam prediction algo" from \cite{alrabeiah_beamprediction_2020}
     \item High mobile users can be tracked through channel info. and channel correlation (cos similarity) with the candidate beams. 
     \item ABF; but what about DBF...potential of existing solution. 
     \item Low mobility users can be clustered using a combination of location and vision assisted techniques. 
 \end{itemize}
 


\begin{itemize}
    \item object detection
    \item Once we have multiple images with single users like the data set used in \cite{alrabeiah_beamprediction_2020}, we can use a similar ResNet-18 like CNN as the one trained in \cite{alrabeiah_beamprediction_2020} to identify the right beam for each of the users.
    \item Once the network is sufficiently trained, i.e., the accuracy on the validation set is above some threshold, we can then use the beam prediction results to cluster users that all identify the same best beam together
\end{itemize}

channel info (very expensive; very accurate)

user location only (might work in LoS setting but cannot generalize). 

BS images only: need for user detection algorithms

BS images + location : Ideal combo?

Argument: with LoS communications, from just the user position , the "best beam" can be determined. 

But, with more complex channels, that is not possible. 

So, what? - Ahan, user location to learn the channel -= then, BS image to learn advanced features that help determine the best beam (highest SINR). Then, combine users!!
